Edge-oriented Implicit Neural Representation with Channel Tuning

Implicit neural representation, which expresses an image as a continuous function rather than a discrete grid form, is widely used for image processing. Despite its outperforming results, there are still remaining limitations on restoring clear shapes of a given signal such as the edges of an image. In this paper, we propose Gradient Magnitude Adjustment algorithm which calculates the gradient of an image for training the implicit representation. In addition, we propose Edge-oriented Representation Network (EoREN) that can reconstruct the image with clear edges by fitting gradient information (Edge-oriented module). Furthermore, we add Channel-tuning module to adjust the distribution of given signals so that it solves a chronic problem of fitting gradients. By separating backpropagation paths of the two modules, EoREN can learn true color of the image without hindering the role for gradients. We qualitatively show that our model can reconstruct complex signals and demonstrate general reconstruction ability of our model with quantitative results.

==> progress_report/5_dataset.tex <==
We select various signal data to perform extensive experiments and demonstrate our approach. 
1) We illustrate the reconstruction performance of \algname~ with ImageNet benchmarks data. Specifically, we choose the images of various characteristics, such as the image with complex patterns, colorful objects, or some local fluctuations. 2) We use DIV2K benchmarks, commonly used dataset for super resolution, to show that \algname~ also has competitive results on single image super resolution task. 3) Not only to the image data, We apply \algname~ to the audio signal data. We follow the audio dataset of \cite{chen2021learning}, the first 7 seconds from Bach's Cello Suite No.1. 


